Search for contact interactions and large extra dimensions in the dilepton channel using proton-proton collisions at $\sqrt{s}$ = 8 TeV with the ATLAS detector

A search is conducted for non-resonant new phenomena in dielectron and dimuon final states, originating from either contact interactions or large extra spatial dimensions. The LHC 2012 proton-proton collision dataset recorded by the ATLAS detector is used, corresponding to 20 fb$^{-1}$ at $\sqrt{s}$ = 8 TeV. The dilepton invariant mass spectrum is a discriminating variable in both searches, with the contact interaction search additionally utilizing the dilepton forward-backward asymmetry. No significant deviations from the Standard Model expectation are observed. Lower limits are set on the $\ell\ell q q$ contact interaction scale $\Lambda$ between 15.4 TeV and 26.3 TeV, at the 95% credibility level. For large extra spatial dimensions, lower limits are set on the string scale $M_{S}$ between 3.2 TeV to 5.0 TeV.

==> author_list.tex <==
\author[13]{T.~Berry}					
\author[24]{M.~Cano Bret}
\author[6]{R.~Daya}				
\author[13]{L.~Duguid}	
%\author[8]{E.~Etzion}  			
\author[9]{F.~Ellinghaus}					
\author[20]{W.~Fedorko}				
\author[18]{D.~Hayden}					
%\author[27]{S.~Heim}	
%\author[1]{T.~Hryn'ova} 			
\author[15]{U.~Klein}
\author[15]{J.~Kretzschmar}  				
\author[9]{S.~Rave}
\author[24]{E.~Rizvi}
\author[13]{G.~Savage}
\author[15]{Y.J.~Schnellbach}
%\author[19]{B.~Stelzer}
%\author[12]{O.~Stelzer-Chilton} 			
\author[21]{T.~Varol}
\author[19]{S.~Viel}
\author[21]{S.~Willocq}	
\author[9]{M.~Zinser}	


%\affil[1]{LAPP Annecy}
%\affil[2]{Universidade Federal do Rio de Janeiro}
%\affil[3]{CEA Saclay} 
%\affil[4]{University of Wisconsin}   
%\affil[5]{Univ. Illinois at Urbana-Champaign} 
\affil[6]{Brandeis University}
%\affil[7]{University of Tokyo}
%\affil[8]{Tel Aviv University}
\affil[9]{Institut fur Physik, Universit\"at Mainz}
%\affil[10]{B.P. Konstantinov Petersburg Nuclear Physics Institute}
%\affil[11]{University of Birmingham}
%\affil[12]{TRIUMF}
\affil[13]{Royal Holloway London}
%\affil[14]{Duke University}
\affil[15]{University of Liverpool}
%\affil[16]{LPSC Grenoble}
%\affil[17]{Oxford University}
\affil[18]{Michigan State University}
\affil[19]{Simon Fraser University}
\affil[20]{University of British Columbia}
\affil[21]{University of Massachusetts, Amherst}
%\affil[22]{Joint Institute for Nuclear Research, Dubna}
%\affil[23]{Max-Planck-Institut f\"ur Physik, M\"unchen}
\affil[24]{Queen Mary University of London}
%\affil[24]{Ludwig-Maximilians-Universit\"at M\"unchen}
%\affil[25]{Boston University}
%\affil[26]{CP3-Origins}
%\affil[27]{University of Pennsylvania}

%%% OLDER AUTHOR LIST BELOW

%\author[30]{A.~A. Abdelalim}
%\author[132]{D.~Adams}
%\author[5]{C.~Amelung}
%%\author[126]{A.~Antonaki}
%\author[9]{T.~Addy}
%\author[1]{L.~Aperio~Bella}
%\author[2]{A.~Asevedo~Nepomuceno}
%%\author[18]{H.~Bachacou}
%\author[28]{M.~A.~Barros do Vale}
%\author[18]{F.~Bauer}
%\author[3]{P.~Bell}
%\author[21]{G.~Bella}
%\author[26]{N.~Benekos}
%\author[17]{T.~Berry}
%%\author[4]{K.~Black}
%\author[6]{N.~Bolnet}
%\author[12]{I.~Boyko}
%\author[4]{J.~Butler}
%\author[7]{E.~Castaneda-Miranda}
%\author[34]{F.~Cerutti}
%\author[6]{L.~Chevalier}
%\author[12]{M.~Chizhov}
%%\author[128]{G.~Choudalakis}
%\author[26]{J.~Coggeshall}
%%\author[37]{K.~Copic}
%%\author[134]{Z.~Czyczula}
%\author[5]{R.~K.~Daya}
%\author[27]{J.~Degenhardt}
%\author[10]{T.~Dohmae}
%\author[17]{L.~Duguid}
%\author[21]{E.~Etzion}
%\author[11]{F.~Ellinghaus}
%%\author[126]{D.~Fassouliotis}
%\author[15]{O.~Fedin}
%\author[16]{W.~Fedorko}
%\author[5]{E.~Fitzgerald}
%\author[7]{L.~R.~Flores-Castillo}
%\author[22]{D.~Fortin}
%\author[3]{S.~Gadomski}
%\author[3]{M.~Goulette}
%\author[6]{P.-F.~Giraud}
%\author[11]{C.~G\"{o}ringer}
%\author[6]{C.~Guyot}
%\author[17]{D.~Hayden}
%\author[16]{S.~Heim}
%\author[27]{M.~Hickman}
%\author[21]{N.~Hod}
%\author[24]{S.~Hou}
%\author[1]{T.~Hryn'ova}
%%\author[131]{A.~Ishikawa}
%\author[27]{B.~Jackson}
%%\author[10]{Y.~Jiang}
%\author[29]{O.~Kortner}
%\author[8]{A.~Kotwal}
%\author[18]{J.~Kretzschmar}
%%\author[126]{C.~Kourkoumelis}
%\author[13]{E.~Laisn\'e}
%\author[13]{F.~Ledroit}
%\author[31]{W.~Liebig}
%\author[26]{T.~Liss}
%%\author[25]{Y.~Liu}
%\author[4]{A.~Long}
%\author[4]{J.~Love}
%\author[30]{P.~Mal}
%\author[15]{V.~Maleev}
%\author[2]{F.~Marroquim}
%\author[6]{H.~Martinez-Bruzual}
%%\author[3]{B.~Martin Dit Latour}
%%\author[6]{N.~Morange}
%\author[3]{K.~Nikolics}
%\author[14]{T.~Nunnemann}
%\author[27]{D.~Olivito}
%%\author[134]{F.~Ould-Saada}
%\author[3]{G.~Pasztor}
%%\author[37]{J.~Parsons}
%%\author[37]{A.~Penson}
%\author[32]{L.~Pontecorvo}
%\author[29]{I.~Potrap}
%%\author[36]{D.~Prieur}
%%\author[133]{J.~Qian}
%\author[33]{M.~Schernau}
%\author[5]{G.~Sciolla}
%\author[18]{Y.-J.~Schnellbach}
%\author[16]{R.~Schwienhorst}
%\author[9]{T.~Shin}
%\author[21]{Y.~Silver}
%\author[15]{V.~Solovyev}
%\author[27]{J.~Stahlman}
%\author[19]{B.~Stelzer}
%\author[22]{O.~Stelzer-Chilton}
%%\author[109]{R.~Stroynowski}
%%\author[8]{S.~Sun}
%%\author[9]{A.~Tetteh}
%\author[27]{E.~Thomson}
%%\author[20]{E.~Thompson}
%\author[16]{K.~Tollefson}
%%\author[20]{N.~van Eldik}
%\author[19]{K.~van Nieuwkoop}
%\author[20]{T.~Varol}
%\author[9]{V.~Vassilakopoulos}
%\author[22,23]{S.~Viel}
%%\author[12]{A.~Vostrikov}
%%\author[27]{P.~Wagner}
%\author[24,25]{H.~Wang}
%%\author[40]{M.~Wielers}
%\author[27]{H.~Williams}
%\author[20]{S.~Willocq}
%\author[7]{S.~L.~Wu}
%\author[3]{X.~Wu}
%%\author[37]{E.~Wulf}
%\author[12]{I.~Yeletskikh}
%\author[5]{S.~Zambito}
%\author[25]{Q.~Zhu}
%%\author[133]{J.~Zhu}
%
%
%\affil[1]{LAPP Annecy}
%\affil[2]{Universidade Federal do Rio de Janeiro}
%\affil[3]{Universit\'e de Gen\`eve}
%\affil[4]{Boston University}
%\affil[5]{Brandeis University}
%\affil[6]{CEA Saclay}
%\affil[7]{University of Wisconsin}
%\affil[8]{Duke University}
%\affil[9]{Hampton University}
%\affil[10]{University of Tokyo}
%\affil[11]{Institut fur Physik, Universitat Mainz, Mainz }
%\affil[12]{Joint Institute of Nuclear Research, Dubna}
%\affil[13]{LPSC Grenoble}
%\affil[14]{Ludwig-Maximilians-Universit\"at M\"unchen}
%\affil[15]{B.P. Konstantinov Petersburg Nuclear Physics Institute}
%\affil[16]{Michigan State University}
%\affil[17]{Royal Holloway London}
%\affil[18]{University of Liverpool}
%\affil[19]{Simon Fraser University}
%\affil[20]{University of Massachusetts, Amherst}
%\affil[21]{Tel Aviv University}
%\affil[22]{TRIUMF}
%\affil[23]{University of British Columbia}
%\affil[24]{Academica Sinica}
%\affil[25]{University of Science \& Technology of China}
%\affil[26]{Univ. Illinois at Urbana-Champaign}
%\affil[28]{Federal University of S$\tilde{a}$o Jo$\tilde{a}$o del Rei (UFSJ)}
%\affil[29]{Max-Planck-Institut f\"ur Physik, M\"unchen}
%\affil[30]{University of Arizona}
%\affil[31]{University of Bergen}
%\affil[32]{INFN Sezione di Roma I}
%\affil[33]{University of California, Irvine}
%\affil[34]{INFN Laboratori Nazionali di Frascati}
%%\affil[109]{Southern Methodist University}
%%\affil[126]{University of Athens}
%%\affil[128]{University of Chicago}
%%\affil[131]{University of Kobe}
%%\affil[132]{Brookhaven National Laboratory}
%%\affil[133]{University of Michigan}
%%\affil[134]{University of Oslo}
%%\affil[36]{University of Pittsburgh}
%%\affil[37]{Columbia University}
%%\affil[40]{Rutherford Appleton Laboratory}
%%\affil[41]{Ludwig-Maximilians-Universit\"at M\"unchen}

%\affil[99]{ATLAS Experiment}

